NLO QCD corrections to tW' and tZ' production in forward-backward asymmetry models

We consider Z' and W' models recently proposed to explain the top forward-backward asymmetry at the Tevatron. We present the next-to-leading order QCD corrections to associated production of such vector bosons together with top quarks at the Large Hadron Collider, for centre-of-mass energies of 7 and 8 TeV. The corrections are significant, modifying the total production cross-section by 30-50%. We consider the effects of the corrections on the top and vector-boson kinematics. The results are directly applicable to current experimental searches, for both the ATLAS and CMS collaborations.

==> TotalCrossSection2.tex <==
\section{Total cross section  for $\mathbf{tW'}$ and $\mathbf{tZ'} $' production}
\label{sec:total}
In this section, we present results for total NLO cross-sections, for the 
process of eq.~(\ref{proc}). For ease of comparison with 
e.g.~\cite{Gresham:2011dg}, we begin by considering the Lagrangian of 
eq.~(\ref{couplings}) with a non-zero coupling between the first and third
generations only. That is, $P_{td}=Q_{tu}=1$ and $P_{ts}=P_{tb}=Q_{tc}=0$.
Furthermore, we fix $g_R=1$, and use default renormalisation and 
factorisation scale choices of $\mu_R=\mu_F=(m_t+m_X)/2$, where $m_X$ is the
mass of the $W'$ or $Z'$ boson, as appropriate, and $m_t=172.5$ GeV is the top
quark mass. We consider the LHC, with a centre of mass energy of 7 TeV.\\

Results for the total cross-section (i.e. the sum of both top and antitop 
production) at LO and NLO are shown for both $Z'$ and $W'$ production in 
tables~\ref{tab:lo-zp}--\ref{tab:nlo-wp}. We show all results using both
CTEQ~\cite{Pumplin:2002vw,Lai:2010vv} and MSTW~\cite{Martin:2009iq} partons, 
where for the latter we calculate the PDF uncertainty using the relevant PDF 
error sets. In all subsequent plots, we show results using MSTW partons unless
otherwise stated. For each result, we also present the scale variation 
uncertainty obtained by varying both $\mu_F$ and $\mu_R$ independently in the 
range $\mu_0/2,2\mu_0$, where $\mu_0$ is the default scale. One sees that the
scale variation uncertainty is reduced at NLO, as expected. Furthermore, the
PDF uncertainty is much smaller than the scale uncertainty. This is also to be
expected, given that the cross-section is dominated by the production of top 
quarks involving a $u$ or $d$ quark in the initial state (for $Z'$ and $W'$
production respectively), namely valence quarks. Furthermore, the heavy nature
of the final state (involving both a top quark and a heavy vector boson) means
that the partons are evaluated at typically high momentum fractions $x$. 
Valence quark distributions at high $x$ are well constrained by global PDF 
fits, hence the small PDF uncertainty in the results of 
tables~\ref{tab:lo-zp}-\ref{tab:nlo-wp}. Plots of the total cross-sections for
$Z'$ and $W'$ production are shown in figures~\ref{fig:zp} and~\ref{fig:wp},
where we have added the PDF and scale uncertainties in quadrature {\bf make 
sure we have done this!}. \\

\begin{table}[h]
\begin{center}
\input{tZp-lo-table}
\end{center}
\caption{Leading order cross sections for $pp \rightarrow tZ'$ at the 7 TeV LHC. \label{tab:lo-zp}}
\end{table}

\begin{table}[h]
\begin{center}
\input{tWp-lo-table}
\end{center}
\caption{Leading order cross sections for $pp \rightarrow tW'$ at the 7 TeV LHC. \label{tab:lo-wp}}
\end{table}

\begin{table}[h]
\begin{center}
\input{tZp-nlo-table}
\end{center}
\caption{Next-to-leading order cross sections for $pp \rightarrow tZ'$ at the 7 TeV LHC. \label{tab:nlo-zp}}
\end{table}

\begin{table}[h]
\begin{center}
\input{tWp-nlo-table}
\end{center}
\caption{Next-to-leading order cross sections for $pp \rightarrow tW'$ at the 7 TeV LHC. \label{tab:nlo-wp}}
\end{table}

\begin{figure}
\begin{center}
\caption{{\bf Put $Z'$ total cross-section fig here.}}
\label{fig:zp}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\caption{{\bf Put $W'$ total cross-section fig here.}}
\label{fig:wp}
\end{center}
\end{figure}

In figures~\ref{fig:wpK} and~\ref{fig:zpK}, we show the $K$-factor for both
$Z'$ and $W'$ production as a function of the mass of the gauge boson $m_X$, 
evaluated according to
\begin{equation}
K=\frac{\sigma_{\rm NLO}}{\sigma_{\rm LO}},
\label{Kfacdef}
\end{equation}
where we have used the results obtained with MSTW partons from 
tables~\ref{tab:lo-zp}-\ref{tab:nlo-wp}. We see that the $K$-factor is sizeable
and increasing with $m_X$. For the values of $m_X$ we consider, the NLO 
corrections range from $\simeq 30\%-50\%$  in both cases. This can be compared
with Standard Model $Wt$ production, for which the $K$-factor is 
$\simeq 25\%$~\cite{Campbell:2005bb,Zhu:2002uj}, subject to an appropriate 
on-shell subtraction formalism being employed to separate the $Wt$ mode from
top pair production. The higher $K$ factor in the present case, and the fact
that the $K$-factor rises with increasing gauge boson mass, have partonic 
origins. As stated above, both $W'$ and $Z'$ production have valence quarks
in the initial state. Furthermore, as $m_X$ increases, these distributions
are probed at typically higher $x$ values, and relatively more so at NLO. 
Given that valence quark distributions remain significant at higher $x$ values,
the $K$-factor is therefore sizable. One expects the opposite trend if sea or 
$b$ quarks are involved in the initial state - there one should see a 
$K$-factor which decreases with increasing $m_X$, due to the sharp fall-off in
the partons as $x\rightarrow 1$. One may verify that this is indeed the case
by studying the results of appendix~\ref{app:othercouplings}, in which we 
consider the coupling of $b$, $s$ and $c$ quarks to the top. Note that are
also extra partonic subchannels which open up at NLO (i.e. the $q\bar{q}$ and
$gg$ initial states), which also act to increase the $K$-factor. \\

From tables~\ref{tab:lo-zp}--\ref{tab:nlo-wp} and 
figures~\ref{fig:zpK}--\ref{fig:wpK}, one sees that the $K$-factor for 
$Z'$ production is slightly larger than that for $W'$ production. This is 
presumably explained by the fact that the former case has $u$ quarks in the 
initial state rather than $d$ quarks, and so the initial state parton
distributions are more strongly peaked at the high $x$ values which are 
typically probed during the current scattering process. We may also note from
figures~\ref{fig:zp} and~\ref{fig:wp} that for both $Z'$ and $W'$ production,
the theoretical uncertainty band for the total NLO cross-section (obtained by
adding the PDF and scale uncertainties in quadrature) lies outside the
corresponding uncertainty band for the LO results. This strongly justifies the
calculation of NLO effects undertaken in this paper, in order to set tight 
bounds on the parameter space of $W'$ and $Z'$ models. \\

\begin{figure}
\begin{center}
\caption{{\bf Put $Z'$ $K$-factor fig here.}}
\label{fig:zpK}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\caption{{\bf Put $W'$ $K$-factor fig here.}}
\label{fig:wpK}
\end{center}
\end{figure}

As well as the total cross-section, it is also interesting to consider the 
fraction of events containing a top quark, rather than an antitop quark (in
the case of $W'$ production, this changes the sign of the accompanying boson. 
This fraction is shown for $Z'$ and $W'$ production in 
figures~\ref{fig:tfracZ} and~\ref{fig:tfracW} respectively, at both LO and NLO.
We see in both cases that the total cross-section is dominated by $t$ quark
production, due to the presence of valence rather than sea quarks in the 
initial state at LO. The fraction is higher for $W'$ rather than $Z'$ 
production, due to the dominance of up quarks over down quarks in the proton.
Note that the fractions increase with the gauge boson mass, reflecting the
fact that the partons are evaluated at higher $x$ values on average as the
gauge boson mass increases, which causes sea-quark dominated processes to
fall off at the expense of those which are dominated by valence quarks.
We may also note that the fraction changes slightly at NLO, and can either 
decrease or increase, depending on the gauge boson mass. This is due to two
competing effects. Firstly, extra partonic subchannels open up at NLO which are
insensitive to the exchange of a top and anti-top quark. This acts to decrease
the fraction of top quark events. Secondly, the partons are evaluated at 
slightly higher $x$ values at NLO compared to LO. This increases the dominance
of valence quark-initiated processes, and acts to increase the proportion of
top quark events. This latter effect wins out at higher gauge boson masses,
as can be seen in both figures~\ref{fig:tfracZ} and~\ref{fig:tfracW}.\\

\begin{figure}
\begin{center}
\caption{{\bf Put $Z'$ top quark fraction fig here.}}
\label{fig:tfracZ}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\caption{{\bf Put $W'$ top quark fraction fig here.}}
\label{fig:tfracW}
\end{center}
\end{figure}

In this section, we have considered a subset of possible couplings in 
eq.~(\ref{couplings}), in particular considering only the $u-t$ and $d-t$
interactions for $W'$ and $Z'$ respectively. In 
appendix~\ref{app:othercouplings} we present tables of results for other
possible choices. Furthermore, in appendix~\ref{app:8TeV}, we present results
for the LHC at 8 TeV. Having discussed the total cross-section results in
detail, we discuss NLO corrections to kinematic distributions of the top quark
and gauge bosons in the following section.


==> tWp-nlo-allckm-table.tex <==
\begin{tabular}{|c||r@{.}l|r@{.}l|}
\hline
$M(W')$\,(GeV) & \multicolumn{2}{|c|}{$\sigma^{\mathrm{CT10}}_{\mathrm{nlo}} (tW')$\,(pb)}& \multicolumn{2}{|c|}{$\sigma^{\mathrm{MSTW\ 2008\ NLO}}_{\mathrm{nlo}} (tW')$\,(pb)}\\ 
\hline 
200 & 73&98 & 76&41 \\ 
300 & 23&75 & 24&43 \\ 
400 & 9&155 & 9&362 \\ 
500 & 3&969 & 4&029 \\ 
600 & 1&870 & 1&882 \\ 
700 & 0&938 & 0&935 \\ 
800 & 0&494 & 0&487 \\ 
900 & 0&270 & 0&263 \\ 
1000 & 0&153 & 0&146 \\ 
1100 & 0&0884 & 0&0834 \\ 
1200 & 0&0523 & 0&0485 \\ 
1300 & 0&0315 & 0&0287 \\ 
1400 & 0&0193 & 0&0172 \\ 
1500 & 0&0119 & 0&0104 \\ 
1600 & 0&00748 & 0&00636 \\ 
1700 & 0&00472 & 0&00391 \\ 
1800 & 0&00301 & 0&00242 \\ 
1900 & 0&00193 & 0&00151 \\ 
2000 & 0&00124 & 0&000940 \\ 
\hline 
\end{tabular} 


==> tWp-tb-nlo-8TeV-table.tex <==
\begin{tabular}{|c||c|c|}
\hline
$M(W')$\,(GeV) & $\sigma^{\mathrm{CT10}}_{\mathrm{nlo}} (tW')$\,(pb)& $\sigma^{\mathrm{MSTW\ 2008\ NLO}}_{\mathrm{nlo}} (tW')$\,(pb)\\ 
\hline 
200 & 6.9323 $^{+0.4447}_{-0.3991}$ (Scale) $^{+0.7435}_{-0.6486}$ (PDF)& 7.4971 $^{+0.4840}_{-0.4233}$ (Scale) $^{+0.3033}_{-0.3871}$ (PDF)\\ 
300 & 2.0429 $^{+0.1194}_{-0.0982}$ (Scale) $^{+0.2815}_{-0.2429}$ (PDF)& 2.1983 $^{+0.1299}_{-0.1022}$ (Scale) $^{+0.1095}_{-0.1369}$ (PDF)\\ 
400 & 0.7359 $^{+0.0402}_{-0.0305}$ (Scale) $^{+0.1249}_{-0.1060}$ (PDF)& 0.7866 $^{+0.0434}_{-0.0339}$ (Scale) $^{+0.0466}_{-0.0569}$ (PDF)\\ 
500 & 0.3007 $^{+0.0155}_{-0.0127}$ (Scale) $^{+0.0611}_{-0.0507}$ (PDF)& 0.3187 $^{+0.0165}_{-0.0147}$ (Scale) $^{+0.0220}_{-0.0262}$ (PDF)\\ 
600 & 0.1344 $^{+0.0065}_{-0.0062}$ (Scale) $^{+0.0321}_{-0.0259}$ (PDF)& 0.1411 $^{+0.0070}_{-0.0071}$ (Scale) $^{+0.0111}_{-0.0130}$ (PDF)\\ 
700 & 0.0643 $^{+0.0030}_{-0.0032}$ (Scale) $^{+0.0179}_{-0.0139}$ (PDF)& 0.0667 $^{+0.0031}_{-0.0036}$ (Scale) $^{+0.0059}_{-0.0068}$ (PDF)\\ 
800 & 0.0325 $^{+0.0015}_{-0.0017}$ (Scale) $^{+0.0104}_{-0.0078}$ (PDF)& 0.0333 $^{+0.0016}_{-0.0019}$ (Scale) $^{+0.0033}_{-0.0037}$ (PDF)\\ 
900 & 0.0171 $^{+0.0008}_{-0.0010}$ (Scale) $^{+0.0063}_{-0.0045}$ (PDF)& 0.0173 $^{+0.0009}_{-0.0011}$ (Scale) $^{+0.0019}_{-0.0021}$ (PDF)\\ 
1000 & 0.0093 $^{+0.0005}_{-0.0006}$ (Scale) $^{+0.0039}_{-0.0027}$ (PDF)& 0.0093 $^{+0.0005}_{-0.0006}$ (Scale) $^{+0.0011}_{-0.0012}$ (PDF)\\ 
1100 & 0.0052 $^{+0.0003}_{-0.0003}$ (Scale) $^{+0.0024}_{-0.0016}$ (PDF)& 0.0051 $^{+0.0003}_{-0.0003}$ (Scale) $^{+0.0007}_{-0.0007}$ (PDF)\\ 
1200 & 0.0030 $^{+0.0002}_{-0.0002}$ (Scale) $^{+0.0016}_{-0.0010}$ (PDF)& 0.0029 $^{+0.0002}_{-0.0002}$ (Scale) $^{+0.0004}_{-0.0004}$ (PDF)\\ 
1300 & 0.0018 $^{+0.0001}_{-0.0001}$ (Scale) $^{+0.0010}_{-0.0006}$ (PDF)& 0.0017 $^{+0.0001}_{-0.0001}$ (Scale) $^{+0.0003}_{-0.0003}$ (PDF)\\ 
1400 & 0.0011 $^{+0.0001}_{-0.0001}$ (Scale) $^{+0.0007}_{-0.0004}$ (PDF)& 0.0010 $^{+0.0001}_{-0.0001}$ (Scale) $^{+0.0002}_{-0.0002}$ (PDF)\\ 
1500 & 0.0006 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0005}_{-0.0003}$ (PDF)& 0.0006 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0001}_{-0.0001}$ (PDF)\\ 
1600 & 0.0004 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0003}_{-0.0002}$ (PDF)& 0.0004 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0001}_{-0.0001}$ (PDF)\\ 
1700 & 0.0002 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0002}_{-0.0001}$ (PDF)& 0.0002 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0000}_{-0.0000}$ (PDF)\\ 
1800 & 0.0002 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0001}_{-0.0001}$ (PDF)& 0.0001 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0000}_{-0.0000}$ (PDF)\\ 
1900 & 0.0001 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0001}_{-0.0001}$ (PDF)& 0.0001 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0000}_{-0.0000}$ (PDF)\\ 
2000 & 0.0001 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0001}_{-0.0000}$ (PDF)& 0.0001 $^{+0.0000}_{-0.0000}$ (Scale) $^{+0.0000}_{-0.0000}$ (PDF)\\ 
\hline 
\end{tabular} 


==> tZp-nlo-allckm-table.tex <==
\begin{tabular}{|c||r@{.}l|r@{.}l|}
\hline
$M(Z')$\,(GeV) & \multicolumn{2}{|c|}{$\sigma^{\mathrm{CT10}}_{\mathrm{nlo}} (tZ')$\,(pb)}& \multicolumn{2}{|c|}{$\sigma^{\mathrm{MSTW\ 2008\ NLO}}_{\mathrm{nlo}} (tZ')$\,(pb)}\\ 
\hline 
200 & 109&1 & 111&9 \\ 
300 & 37&53 & 38&44 \\ 
400 & 15&37 & 15&72 \\ 
500 & 7&038 & 7&181 \\ 
600 & 3&484 & 3&547 \\ 
700 & 1&829 & 1&857 \\ 
800 & 1&005 & 1&016 \\ 
900 & 0&572 & 0&576 \\ 
1000 & 0&335 & 0&336 \\ 
1100 & 0&201 & 0&200 \\ 
1200 & 0&123 & 0&122 \\ 
1300 & 0&0766 & 0&0752 \\ 
1400 & 0&0483 & 0&0470 \\ 
1500 & 0&0308 & 0&0297 \\ 
1600 & 0&0198 & 0&0189 \\ 
1700 & 0&0129 & 0&0122 \\ 
1800 & 0&00841 & 0&00784 \\ 
1900 & 0&00552 & 0&00509 \\ 
2000 & 0&00364 & 0&00331 \\ 
\hline 
\end{tabular} 


==> tZp-table.tex <==
\begin{tabular}{|c||r@{.}lll|r@{.}lll|}
\hline
$M(W')$\,(GeV) & \multicolumn{4}{|c|}{$\sigma^{\mathrm{CT10}}_{\mathrm{nlo}} (tW')$\,(pb)}& \multicolumn{4}{|c|}{$\sigma^{\mathrm{MSTW\ 2008\ NLO}}_{\mathrm{nlo}} (tW')$\,(pb)}\\ 
\hline 
200 & 55&63 & $^{+ 3.68}_{- 4.04}$ & $^{+ 2.06}_{- 2.66}$& 57&10 & $^{+ 3.93}_{- 4.28}$ & $^{+ 0.53}_{- 0.87}$\\ 
300 & 18&48 & $^{+ 1.22}_{- 1.40}$ & $^{+ 0.83}_{- 1.00}$& 18&83 & $^{+ 1.29}_{- 1.47}$ & $^{+ 0.21}_{- 0.34}$\\ 
400 & 7&315 & $^{+0.492}_{-0.580}$ & $^{+0.401}_{-0.450}$& 7&398 & $^{+0.517}_{-0.605}$ & $^{+0.103}_{-0.159}$\\ 
500 & 3&241 & $^{+0.226}_{-0.268}$ & $^{+0.216}_{-0.225}$& 3&251 & $^{+0.235}_{-0.277}$ & $^{+0.056}_{-0.082}$\\ 
600 & 1&555 & $^{+0.112}_{-0.134}$ & $^{+0.122}_{-0.123}$& 1&546 & $^{+0.117}_{-0.137}$ & $^{+0.033}_{-0.045}$\\ 
700 & 0&792 & $^{+0.060}_{-0.071}$ & $^{+0.073}_{-0.070}$& 0&780 & $^{+0.061}_{-0.072}$ & $^{+0.020}_{-0.026}$\\ 
800 & 0&423 & $^{+0.033}_{-0.039}$ & $^{+0.046}_{-0.042}$& 0&411 & $^{+0.034}_{-0.039}$ & $^{+0.013}_{-0.015}$\\ 
900 & 0&234 & $^{+0.019}_{-0.022}$ & $^{+0.029}_{-0.026}$& 0&225 & $^{+0.019}_{-0.022}$ & $^{+0.008}_{-0.009}$\\ 
1000 & 0&134 & $^{+0.011}_{-0.013}$ & $^{+0.019}_{-0.016}$& 0&127 & $^{+0.011}_{-0.013}$ & $^{+0.005}_{-0.006}$\\ 
1100 & 0&0781 & $^{+0.0069}_{-0.0080}$ & $^{+0.0127}_{-0.0103}$& 0&0729 & $^{+0.0068}_{-0.0077}$ & $^{+0.0034}_{-0.0037}$\\ 
1200 & 0&0466 & $^{+0.0043}_{-0.0049}$ & $^{+0.0086}_{-0.0067}$& 0&0428 & $^{+0.0041}_{-0.0047}$ & $^{+0.0022}_{-0.0024}$\\ 
1300 & 0&0283 & $^{+0.0027}_{-0.0031}$ & $^{+0.0059}_{-0.0044}$& 0&0255 & $^{+0.0026}_{-0.0029}$ & $^{+0.0015}_{-0.0016}$\\ 
1400 & 0&0174 & $^{+0.0017}_{-0.0019}$ & $^{+0.0041}_{-0.0030}$& 0&0154 & $^{+0.0016}_{-0.0018}$ & $^{+0.0010}_{-0.0010}$\\ 
1500 & 0&0108 & $^{+0.0011}_{-0.0012}$ & $^{+0.0029}_{-0.0020}$& 0&00940 & $^{+0.00102}_{-0.00112}$ & $^{+0.00066}_{-0.00067}$\\ 
1600 & 0&00683 & $^{+0.00073}_{-0.00081}$ & $^{+0.00202}_{-0.00137}$& 0&00578 & $^{+0.00065}_{-0.00071}$ & $^{+0.00044}_{-0.00045}$\\ 
1700 & 0&00434 & $^{+0.00048}_{-0.00053}$ & $^{+0.00143}_{-0.00094}$& 0&00358 & $^{+0.00042}_{-0.00045}$ & $^{+0.00030}_{-0.00030}$\\ 
1800 & 0&00277 & $^{+0.00032}_{-0.00035}$ & $^{+0.00102}_{-0.00065}$& 0&00223 & $^{+0.00027}_{-0.00029}$ & $^{+0.00020}_{-0.00020}$\\ 
1900 & 0&00178 & $^{+0.00021}_{-0.00023}$ & $^{+0.00073}_{-0.00045}$& 0&00139 & $^{+0.00017}_{-0.00018}$ & $^{+0.00013}_{-0.00013}$\\ 
2000 & 0&00115 & $^{+0.00014}_{-0.00015}$ & $^{+0.00052}_{-0.00031}$& 0&000874 & $^{+0.000113}_{-0.000118}$ & $^{+0.000090}_{-0.000089}$\\ 
\hline 
\end{tabular} 

